FileInsurer: A Scalable and Reliable Protocol for Decentralized File Storage in Blockchain

With the development of blockchain applications, the requirements for file storage in blockchain are increasing rapidly. Many protocols, including Filecoin, Arweave, and Sia, have been proposed to provide scalable decentralized file storage for blockchain applications. However, the reliability is not well promised by existing protocols. Inspired by the idea of insurance, we innovatively propose a decentralized file storage protocol in blockchain, named as FileInsurer, to achieve both scalability and reliability. While ensuring scalability by distributed storage, FileInsurer guarantees reliability by enhancing robustness and fully compensating for the file loss. Specifically, under mild conditions, we prove that no more than 0.1\% value of all files should be compensated even if half of the storage collapses. Therefore, only a relatively small deposit needs to be pledged by storage providers to cover the potential file loss. Because of lower burdens of deposit, storage providers have more incentives to participate in the storage network. FileInsurer can run in the top layer of the InterPlanetary File System (IPFS), and thus it can be directly applied in Web 3.0, Non-Fungible Tokens, and Metaverse.

==> code/auto_checkalloc_detail.tex <==
\begin{figure}[htbp]
\begin{algorithm}[H]
\caption{\textsf{Auto} protocol}
\footnotesize
\setstretch{.9}
\textsf{Auto\_CheckAlloc}
\begin{itemize}
    \item \textit{Inputs.} file descriptor $f$
    \item \textit{Goal.} check if file $f$ is already confirmed by all of the selected sectors
\end{itemize}
\begin{algorithmic}
\State $count \gets 0$
\For{$i \in [f.cp]$}
    \State let $entry[i]$ be a reference of $\textsf{allocTable}[f,i]$
\EndFor
\For{$i \in [f.cp]$}
    \If{$entry[i].state \neq \texttt{confirm}$ and $entry[i].state \neq \texttt{corrupted}$}
        \State report that the client failed to upload the file $f$
        \For{$i \in [f.cp]$}
            \State remove $(f,i)$ from \textsf{allocTable}
        \EndFor
        \State remove $f$ from the network
    \EndIf
\EndFor
\For{$i \in [f.cp]$}
    \If{$entry[i].state = \texttt{confirm}$}
        \State $entry[i].prev \gets entry[i].next$
        \State $entry[i].next \gets \textbf{null}$
        \State $entry[i].last \gets Now$
        \State $entry[i].state \gets \texttt{normal}$
    \Else
        \State $entry[i].prev \gets \textbf{null}$
        \State $entry[i].next \gets \textbf{null}$
        \State $entry[i].last \gets -1$
        \State $entry[i].state \gets \texttt{broken}$
    \EndIf
\EndFor
\State $f.cntdown\gets SampleIndex(ProofCycle)$
\State add $CheckProof(f)$ to $\textsf{pendingList}[Now+ProofCycle]$
\State report that the client succeed to upload the file $f$
\end{algorithmic}
\end{algorithm}
\caption{}
\label{auto:checkallocdetail}
\end{figure}

==> code/auto_checkproof_detail.tex <==
\begin{figure}[htbp]
\begin{algorithm}[H]
\caption{\textsf{Auto} protocol}
\footnotesize
\setstretch{.9}
\textsf{Auto\_CheckProof}
\begin{itemize}
    \item \textit{Inputs.} file descriptor $f$
    \item \textit{Goal.} check that all storage locations of file $f$ are working
\end{itemize}
\begin{algorithmic}
\If{the client of file $f$ has does not have enough tokens to pay the rent for the next cycle}
    \State $f.state \gets \texttt{discard}$
    \State report that file $f$ is discarded due to insufficient rent
\EndIf
\If{$f.state = \texttt{normal}$}
    \State deduct the client's rent for the next cycle
    \For{$i \in [f.cp]$}
        \State let $entry$ be a reference of $\textsf{allocTable}[f,i]$
        \If{$entry.prev$ is not corrupted}
            \If{$entry.last < Now - ProofDeadline$}
                \State confiscate the deposit of $s$
                \State mark and report that $s$ is corrupted
            \ElsIf{$entry.last < Now - ProofDue$}
                \State punish $entry.prev$
            \Else
                \State pay the owner of $s$ rent from the previous period
            \EndIf
        \EndIf
    \EndFor
\EndIf
\If{$f.state=\texttt{discard}$}
    \For{$i \in [f.cp]$}
        \State remove $(f,i)$ from \textsf{allocTable}
    \EndFor
    \State remove $f$ from the network
\ElsIf{$\forall j, entry[j].prev$ is corrupted}
    \State report that file $f$ is lost
    \State compensate to the client
    \For{$i \in [f.cp]$}
        \State remove $(f,i)$ from \textsf{allocTable}
    \EndFor
    \State remove $f$ from the network
\Else
    \State add $CheckProof(f)$ to $\textsf{pendingList}[Now+ProofCycle]$
    \State $f.cntdown-=1$
    \If{$f.cntdown=0$}
        \State $i\gets RandomIndex(f)$
        \State \textbf{call} $Refresh(f,i)$
    \EndIf
\EndIf
\end{algorithmic}
\end{algorithm}
\caption{}
\label{auto:checkproofdetail}
\end{figure}

==> code/auto_refresh_detail.tex <==
\begin{figure}[htbp]
\begin{algorithm}[H]
\caption{\textsf{Auto} protocol}
\footnotesize
\setstretch{.9}
\textsf{Auto\_Refresh}
\begin{itemize}
    \item \textit{Inputs.} file descriptor $f$ and index $i$
    \item \textit{Goal.} change one of the storage places of file $f$ to random sectors
\end{itemize}
\begin{algorithmic}
\State $s\gets RandomSector()$
\If {$s.freeCap\geq f.size$}
    \State let $entry$ be a reference of $\textsf{allocTable}[f,i]$
    \State $entry.next \gets s$
    \State $entry.state \gets \texttt{alloc}$
    \State $t \gets Now+DelayPerSize\times f.size$
    \State add $CheckRefresh(f,i)$ to $\textsf{pendingList}[t]$
\Else
    \State $f.cntdown\gets SampleIndex(ProofCycle)$
\EndIf
\end{algorithmic}

\hspace*{\fill}

\textsf{Auto\_CheckRefresh}
\begin{itemize}
    \item \textit{Inputs.} file descriptor $f$ and index $i$
    \item \textit{Goal.} check whether the last refresh for file $f$ is confirmed
\end{itemize}
\begin{algorithmic}
    \State let $entry$ be a reference of $\textsf{allocTable}[f,i]$
    \If{$entry.state=\texttt{confirm}$}
        \State $entry.prev\gets entry.next$
        \State $entry.next\gets \textbf{null}$
        \State $entry.last\gets Now$
        \State $f.cntdown\gets SampleIndex(ProofCycle)$
    \Else
        \State punish $entry.next$
        \For{$j \in [f.cp]$}
            \State punish $\textsf{allocTable}[f,j].prev$
        \EndFor
        \State \textbf{call} $Refresh(f,i)$ 
    \EndIf
\end{algorithmic}
\end{algorithm}
\caption{}
\label{auto:refreshdetail}
\end{figure}

==> code/file_client_detail.tex <==
\begin{figure}[htbp]
\begin{algorithm}[H]
\caption{\textsf{File} protocol: client part}
\footnotesize
\setstretch{.9}
\textsf{File\_Add}
\begin{itemize}
    \item \textit{Inputs.} the size of the file $sz$, the value of the file $val$ and the merkle root of the file $rt$
    \item \textit{Goal.} generate the file descriptor for the file and allocate $k$ sectors to it for storage
\end{itemize}
\begin{algorithmic}
\State $f\gets$ \textbf{new} \textsf{fileDescriptor}
\State $f.size\gets sz$
\State $f.value\gets val$
\State $f.merkleRoot\gets rt$
\State $f.state\gets \texttt{normal}$
\State $f.cp\gets CalcCopyCnt(val)$
\State $f.cntdown\gets -1$
\For{$i \in [f.cp]$}
    \State $\textsf{allocTable}[f,i] \gets \textbf{new } allocEntry()$
    \State let $entry$ be a reference of $\textsf{allocTable}[f,i]$
    \State $s\gets RandomSector()$
    \If {$s.freeCap\geq f.size$}
        \State $entry.prev=\textbf{null}$
        \State $entry.next=s$
        \State $entry.last=-1$
        \State $entry.state=\texttt{alloc}$
    \Else
        \State $entry.prev=\textbf{null}$
        \State $entry.next=\textbf{null}$
        \State $entry.last=-1$
        \State $entry.state=\texttt{corrupted}$
        \State \textbf{}        
    \EndIf
\EndFor
\State $t \gets Now+DelayPerSize\times f.size$
\State add $CheckAlloc(f)$ to $\textsf{pendingList}[t]$
\end{algorithmic}

\hspace*{\fill}

\textsf{File\_Discard}
\begin{itemize}
    \item \textit{Inputs.} a file descriptor $f$
    \item \textit{Goal.} discard file $f$
\end{itemize}
\begin{algorithmic}
    \State $f.state \gets \texttt{discard}$
\end{algorithmic}

\end{algorithm}
\caption{\textbf{\textsf{File} Protocol}: client part}
\label{file:clientdetail}
\end{figure}

==> code/file_provider_detail.tex <==
\begin{figure}[htbp]
\begin{algorithm}[H]
\caption{\textsf{File} protocol: provider part}
\footnotesize
\setstretch{.9}
\textsf{File\_Confirm}
\begin{itemize}
    \item \textit{Inputs.} file descriptor $f$, index $i$ and sector $s$
    \item \textit{Goal.} confirm that a selected sector begins to store a specific file
\end{itemize}
\begin{algorithmic}
\State check the request is from the owner of sector $s$
\State let $entry$ be a reference of $\textsf{allocTable}[f,i]$
\State ensure $entry.next = s$ and $entry.state = \texttt{alloc}$ 
\State $entry.state \gets \texttt{confirm}$
\end{algorithmic}

\hspace*{\fill}

\textsf{File\_Prove}
\begin{itemize}
    \item \textit{Inputs.} file descriptor $f$, index $i$, sector $s$ and proof $\pi$
    \item \textit{Goal.} verify that a selected sector is storing specific file
\end{itemize}
\begin{algorithmic}
\State ensure the input request has been signed by the owner of sector $s$
\State let $entry$ be a reference of $\textsf{allocTable}[f,i]$
\State ensure $entry.prev = s$
\State verify $\pi$ is a valid proof at time $\pi.t$
\State $entry.last \gets \pi.t$
\end{algorithmic}
\end{algorithm}
\caption{}
\label{file:providerdetail}
\end{figure}

==> code/sector_detail.tex <==
\begin{figure}[htbp]
\begin{algorithm}[H]
\caption{\textsf{Sector} protocol}
\footnotesize
\setstretch{.9}
\textsf{Sector\_Register}
\begin{itemize}
    \item \textit{Inputs.} capacity $cap$ and owner $own$
    \item \textit{Goal.} register a new sector on the network
\end{itemize}
\begin{algorithmic}
\State the owner pledges deposit proportional to the sector size
\State $s\gets \textbf{new } sector$
\State $s.owner\gets own$
\State $s.id\gets nextid(own)$
\State $s.capacity\gets cap$
\State $s.freeCap\gets cap$
\State $s.state\gets \texttt{normal}$
\end{algorithmic}

\hspace*{\fill}

\textsf{Sector\_Disable}
\begin{itemize}
    \item \textit{Inputs.} sector $s$
    \item \textit{Goal.} mark the sector as disabled
\end{itemize}
\begin{algorithmic}
    \State $s.state \gets \texttt{disable}$
\end{algorithmic}
\end{algorithm}
\caption{}
\label{sector:detail}
\end{figure}
